Towards Human Computable Passwords

An interesting challenge for the cryptography community is to design authentication protocols that are so simple that a human can execute them without relying on a fully trusted computer. We propose several candidate authentication protocols for a setting in which the human user can only receive assistance from a semi-trusted computer --- a computer that stores information and performs computations correctly but does not provide confidentiality. Our schemes use a semi-trusted computer to store and display public challenges $C_i\in[n]^k$. The human user memorizes a random secret mapping $\sigma:[n]\rightarrow\mathbb{Z}_d$ and authenticates by computing responses $f(\sigma(C_i))$ to a sequence of public challenges where $f:\mathbb{Z}_d^k\rightarrow\mathbb{Z}_d$ is a function that is easy for the human to evaluate. We prove that any statistical adversary needs to sample $m=\tilde{\Omega}(n^{s(f)})$ challenge-response pairs to recover $\sigma$, for a security parameter $s(f)$ that depends on two key properties of $f$. To obtain our results, we apply the general hypercontractivity theorem to lower bound the statistical dimension of the distribution over challenge-response pairs induced by $f$ and $\sigma$. Our lower bounds apply to arbitrary functions $f $ (not just to functions that are easy for a human to evaluate), and generalize recent results of Feldman et al. As an application, we propose a family of human computable password functions $f_{k_1,k_2}$ in which the user needs to perform $2k_1+2k_2+1$ primitive operations (e.g., adding two digits or remembering $\sigma(i)$), and we show that $s(f) = \min\{k_1+1, (k_2+1)/2\}$. For these schemes, we prove that forging passwords is equivalent to recovering the secret mapping. Thus, our human computable password schemes can maintain strong security guarantees even after an adversary has observed the user login to many different accounts.

==> OldSecurityProofs.tex <==


\begin{definition} \label{def:HardToPredict2}
We say that a function $f$ is $\paren{\delta_1,\delta_2}$---hard to predict if $\forall \sigma,\sigma' \in\mathbb{Z}_d^n$ s.t. $\sigma$ is $\delta_1$-balanced and $\sigma'$ is not $\delta_1$-correlated with $\sigma$ we have
 \[ \Pr_{C \sim X_k}\left[f\paren{\sigma\paren{C}} = f \paren{\sigma'\paren{C}} \right] \leq \frac{1}{d}+\delta_2   \ . \]
\end{definition}

Intuitively, Definition \ref{def:HardToPredict2} says that if the mappings $f\paren{\sigma'\paren{C}}$ is a good predictor of $f\paren{\sigma'\paren{C}}$ then the mappings $\sigma$ and $\sigma'$ must be related. This is a reasonable property to expect of a secure human computable function. For example, consider a function $f$ is highly correlated with a constant function ($f$ will clearly not be a secure human computable function as all of the passwords are likely to match one fixed string). We note that $f\paren{\sigma'\paren{C}}$ will always be a good predictor of $f\paren{\sigma\paren{C}}$ even for unrelated mappings. Claim \ref{claim:FamilyIsHardToPredict} says that our family of human computable functions satisfies this property.


\newcommand{\factCandidateOneIsHard}{$f_{2,2}$ is $\paren{0.01,0.045}$---hard to predict.}
\begin{fact} \label{fact:Candidate1Hard}
\factCandidateOneIsHard
\end{fact}

Similarly, Fact \ref{fact:Candidate2Hard} together with Theorem \ref{thm:secFinal} provides strong evidence that $f_{1,3}$ is $\UFRCASecure{n}{m}{t}{\delta}$ for $m = \tilde{\Omega}\paren{n^{2}}$. The proof of Facts \ref{fact:Candidate1Hard} and \ref{fact:Candidate2Hard} can be found in the appendix.

\newcommand{\factCandidateTwoHard}{$f_{1,3}$ is $(0.01,0.01)$---hard to predict.}
\begin{fact} \label{fact:Candidate2Hard}
\factCandidateTwoHard
\end{fact}




\newcommand{\lemmaSecurity}{Let $f$ be $\paren{\delta_1,\delta_2}$---hard to predict, let $\sigma \sim \mathbb{Z}_d^n$ denote the secret mapping, let $\epsilon > 0$ be any constant and suppose that we are given labels $\ell_C \in \mathbb{Z}_d$ for every $C \in X_k$ s.t 
\[ \Pr_{C \sim X_k}\left[ f\paren{\sigma\paren{C}} = \ell_C  \right] \geq \frac{1}{d} + \delta_2 + \epsilon \ . \] 
There is a polynomial time algorithm (in $n,1/\epsilon,1/\delta_2$) that with high probability finds a mapping $\sigma' \in \mathbb{Z}_d^n$ such that $\sigma'$ is $\delta_1$-correlated with $\sigma$ provided that $\sigma$ is $\delta_1$-balanced.
}
Theorem \ref{lemma:security} implies that predicting $f\paren{\sigma\paren{C}}$ is just as hard as finding a mapping $\sigma'$ that is correlated with $\sigma$. 
Corollary \ref{cor:security} says that any statistical adversary needs to see at least $\tilde{\Omega}\paren{n^{r(f)/2}}$ example challenge response pairs before it can accurately guess the value of $f\paren{\sigma\paren{C}}$ for a randomly chosen challenge $C \in X_k$. Corollary \ref{cor:security} follows easily from Theorems \ref{lemma:security} and \ref{thm:SecurityLowerBound}. 


\begin{theorem}\label{lemma:security}
\lemmaSecurity
\end{theorem}

We will briefly overview the proof of Theorem \ref{lemma:security} before presenting the formal proof. We first randomly partition $[n]$ into $n/\tau$ parts $S_1,...,S_{n/\tau}$ where $\tau = \tilde{O}\paren{\log n}$. For each set $S_i$, we can check all of the mappings $\sigma_i'\paren{S_i} \in \mathbb{Z}_d^\tau$ to find the one that is consistent with the most noisy labels $\ell_C$ for each $C \in S_i$. With high probability for each set $S_i$ we have
\[ \Pr\left[\ell_C = f\paren{\sigma\paren{C}}~\vline~C\subset S_i \right] \approx \Pr\left[\ell_C = f\paren{\sigma\paren{C}}\right] \ .\]
Because $f$ is $\paren{\delta_1,\delta_2}$---hard to guess this means that for each $i$ the strings $\sigma_i'\paren{S_i} \in \mathbb{Z}_d^\tau$ and  $\sigma\paren{S_i} \in \mathbb{Z}_d^\tau$ are $\delta_2$-correlated. We combine each of the $\sigma_i'$ mappings to construct a mapping $\sigma' \in \mathbb{Z}_d^n$ that is $\delta_2$-correlated with $\sigma$.

\begin{proofof}{Theorem \ref{lemma:security}}
Let $\sigma \in  \mathbb{Z}_d^n$ be given such that $\sigma$ is $\delta_1$-balanced (e.g.,  $\frac{d-1}{d}-\delta_1 \leq \max_{i\in \mathbb{Z}_d} \paren{\frac{H\paren{\sigma,\vec{i}}}{n}} \leq \frac{d-1}{d}+\delta_1 $. 

We set $\tau = \frac{2}{\epsilon^2} \ln\paren{T}$ and select clauses $C^j_1,\ldots C^j_\tau$ at random for $j \in [y]$. Then by Chernoff bounds
\begin{eqnarray*}
\Pr\left[ \left|\left\{i~\vline~\ell_{C^j_i} = f\paren{\sigma\paren{C^j_i}} \right\} \right| \leq \frac{\tau}{d} + \tau\delta_2\right] &\leq& \exp\paren{2\frac{2}{\epsilon^2}\ln{\paren{T}}\epsilon^2}  \\
&=& \exp\paren{4\ln{\paren{T}}}  \\
&=& \frac{1}{T^4}  \ .  
\end{eqnarray*}
Let $T = n$, set $S^j = \bigcup_{i=1}^\tau C^j_i$, and define $BAD^j$ to be the event that \[ \frac{\left|\left\{C\in X_k~\vline~C \subseteq S^j \wedge \ell_{C} = f\paren{\sigma\paren{C}} \right\} \right|}{\left|\left\{C\in X_k~\vline ~C \subseteq S^j\right\}\right|} \leq \frac{1}{d} + \delta_2 \ .\]  
By the union bound 
\begin{eqnarray*}
\Pr\left[BAD^i \right] &\leq&   \binom{\frac{2 k \ln T}{ \epsilon^2}}{k} \frac{1}{T^4} \\
&\leq& \frac{2^kk^k \ln^k T}{\delta^{2k}T^4} \\ 
&\leq& \frac{1}{n^3} \ .
\end{eqnarray*}
If we set $y= O\paren{n \log n}$ then with high probability $\bigcup_{j=1}^y S^j = [n]$. By applying the union bound again we have
\[\Pr\left[\exists j \in [y]. BAD^j\right] \leq \frac{1}{n^{1.5}} \ . \]
Now for each $j \in [y]$ we can enumerate over all $n^{O\paren{(2k\ln d)/\delta_2^2}}$ mappings $\sigma^j\in  \mathbb{Z}_d^{\left|S^j \right|}$ to find one that satisfies
\[  \frac{\left|\left\{C\in X_k~\vline~C \subseteq S^j \wedge \ell_{C} = f\paren{\sigma^j\paren{C}} \right\} \right|}{\left|\left\{C\in X_k~\vline ~C \subseteq S^j\right\}\right|} \geq \frac{1}{d} + \delta_2 \ ,\]
 in polynomial time. Because $f$ is $\paren{\delta_1,\delta_2}$-hard to predict $\sigma^j\paren{S_j}$ must be $\delta_1$-correlated with $\sigma\paren{S_j}$ (e.g.,  $\frac{H\paren{\sigma\paren{S^j},\sigma^j\paren{S^j}}}{\left|S^j \right|} \leq \frac{d-1}{d}-\delta_1$).  Now we can find $\sigma'$ s.t. $H\paren{\sigma,\sigma'} \leq \frac{d-1}{d} - \delta_1$ by combining the $\sigma^i$'s.
\end{proofof}



\begin{corollary} \label{cor:security}
Let $\epsilon > 0$ be any constant and let $\Adversary$ be any statistical adversary that outputs labels $\ell_C$ for each clause $C \in X_k$ after making at most $m = o\paren{\frac{n^{r(f)/2}}{\log^{r(f)} n}}$ queries to $\MSAMPLE\paren{n^{r(f)/2}}$. If $f$ is $\paren{\delta_1,\delta_2}$---hard to predict then with probability $1-o(1)$ we have
\[ \Pr_{\substack{\sigma\sim\mathbb{Z}_d^n\\C \sim X_k}}\left[ f\paren{\sigma\paren{C}} = \ell_C  \right] \leq \frac{1}{d} + \delta_2 +\epsilon \ . \] 
\end{corollary}



\begin{theorem} \label{thm:secFinalOld}
Suppose that $f$ is $\paren{\delta_1,\delta_2}$---hard to predict, but that $f$ is not $\UFRCASecure{n}{m}{t}{\delta}$ for $\delta > \paren{\frac{1}{d}+\delta_2+\epsilon}^t$. Then there is a probabilistic polynomial time algorithm (in $n$, $m$, $1/\delta_1$, $1/\delta_2$, $1/\epsilon$) that extracts a string $\sigma' \in \mathbb{Z}_d^n$ that is $c$-correlated with $\sigma$ after seeing $\tilde{O}\paren{m}$ examples, where $c > 0$ is a constant.
\end{theorem}

\begin{proofof}{Theorem \ref{thm:secFinalOld}} (sketch)
We first partition $X_k$ into $T = O\paren{\frac{\log\left|X_k\right|}{\epsilon}}$ sets $S_1,\ldots,S_T$ of equal size. We let $U_i^j$ denote the set of unlabeled clauses from $S_j$ at time $i$. Initially, $U_0^j = S_j$. During step $i$ we draw $mT$ labeled examples $\paren{C_1^{i,j},f\paren{\sigma\paren{C_1^{i,j}}}},\ldots,\paren{C_m^{i,j},f\paren{\sigma\paren{C_m^{i,j}}}} \sim Q^f_\sigma$ and $t$ labeled examples $\paren{\hat{C}_1^{i,j},f\paren{\sigma\paren{\hat{C}_1^{i,j}}}},\ldots,\paren{\hat{C}_t^{i,j},f\paren{\sigma\paren{\hat{C}_t^{i,j}}}} \sim Q^f_\sigma$. For each clause $C \in U_i$ we select $k_C \sim [t]$ uniformly at random.  We set \[U_{i+1}^j = \left\{C \in U_i^j~\vline~\mathcal{P}_{b,k_C,\hat{C}_1^{i,j},\ldots,\hat{C}_t^{i,j}}\paren{C}=\bot \right\} \ ,\] and we set \[\ell_C = \mathcal{P}_{b,k_C,\hat{C}_1^{i,j},\ldots,\hat{C}_t^{i,j}}\paren{C} \, \] for all $C \in U_i^j\backslash U_{i+1}^j$. Here, $b = \Adversary_{C_1^i,\ldots,C_m^i}$. 

We first argue that $O\paren{\frac{\ln \left|X_k\right|}{\ln\paren{\frac{t}{t-1}} }}$ rounds suffice to label every clause $C \in X_k$. Notice that $\forall C \in X_k$ we have
\[\Pr_{\substack{j \sim[t]\\C_1^{i,j},\ldots,C_m^{i,j}\sim X_k\\\hat{C}_1^{i,j},\ldots,\hat{C}_{t}^{i,j}\sim X_k}}\left[\mathcal{P}_{b,j,\hat{C}_1^{i,j},\ldots,\hat{C}_t^{i,j}}\paren{C} \neq \bot \right] \geq \Pr_{j\sim[t]}[j=1] =  \frac{1}{t} \ . \]
The probability that a clause $C$ hasn't been labeled after $i$ rounds is at most $\paren{1-\frac{1}{t}}^i$. By union bounds the probability that any clause is unlabeled is at most $\left|X_k\right|\paren{1-\frac{1}{t}}^i$ so after $i=O\paren{\frac{\ln \left|X_k\right|}{\ln\paren{\frac{t}{t-1}} }}$ rounds we will have $U_i^j = \emptyset$ for all $j \in [T]$. \\
We now argue that with high probability we label at least $\frac{1}{d}+\delta+\epsilon/2$ clauses correctly. Formally, let \[x_i = \left|\left\{C \in S_i~\vline~\ell_C = f\paren{\sigma\paren{C}} \right\} \right| \ ,\]
denote the number of clauses in $S_i$ labeled correctly.
Notice that the random variables are independent, and by Claim \ref{claim:secFinal} we have \[\mathbb{E}\left[ \sum_{i=1}^T \frac{x_i}{\left|X_k\right|}\right] \geq \frac{1}{d}+\delta+\epsilon  \ . \]
Now by Chernoff Bounds it follows that with probability $1-o(1)$ 
\[\sum_{i=1}^T \frac{x_i}{\left|X_k\right|} \geq \frac{1}{d}+\delta+\epsilon/2 \ , \]
so we can apply Lemma \ref{lemma:security} to obtain the desired result.

\end{proofof}


\section{Proofs of Claims and Facts} \label{apdx:ProofOfClaims}


\begin{reminderfact}{\ref{fact:Candidate1Hard}}
\factCandidateOneIsHard
\end{reminderfact}

\begin{proofof}{Fact \ref{fact:Candidate1Hard}}
Let $\sigma,\sigma'\in \mathbb{Z}_{10}^n$ be given.  We assume that $\sigma$ is $\paren{\frac{1}{100}}$-balanced and that $\sigma$ and $\sigma'$ are not $\paren{\frac{1}{100}}$-correlated. This means that $\frac{9}{100} \leq \max_{i\in \mathbb{Z}_{10}} \paren{n-\frac{H\paren{\sigma,\vec{i}}}{n}} \leq \frac{11}{100}$ and   $\paren{1-\frac{H\paren{\sigma,\sigma'}}{n}} < \frac{11}{100}$. It suffices to show that  \[\Pr_{C=\paren{x_1,\ldots,x_{14}} \sim X_{14}}\left[ f\paren{\sigma\paren{C}} 
 = f\paren{\sigma '\paren{C}} \right] \leq \frac{145}{1000} \ . \]

For $j \in \mathbb{Z}_{10}$ we let $p_j = \frac{n-H\paren{\sigma_j,\sigma '}}{n}$ where $\sigma_j\paren{i} = \paren{\sigma\paren{i}+j \mod {10}}$. In particular, $p_{0} = \frac{n-H\paren{\sigma,\sigma '}}{n}$ denotes the probability that $\sigma(i) = \sigma '(i)$ for a random index $i \sim [n]$. By assumption $p_{0} \leq \frac{1}{10}+\frac{1}{100}$. We have

\begin{eqnarray*}
&& \Pr_{C=\paren{x_1,\ldots,x_{14}} \sim X_{14}}\left[ f_1\paren{\sigma\paren{C}} 
 = f_1\paren{\sigma '\paren{C}} \right] \\ &=& \paren{\sum_{\substack{i,j\in \mathbb{Z}_{10} \\ i+j\equiv 0 \mod{10}}} p_ip_j } \Pr_{C=\paren{x_1,\ldots,x_{14}} \sim X_{14}}\left[ f_1\paren{\sigma\paren{C}} = f_1\paren{\sigma '\paren{C}}~\vline ~  \sigma\paren{x_{11}} + \sigma\paren{x_{12}} \equiv \sigma'\paren{x_{11}}+\sigma'\paren{x_{12}} \mod{10}  \right] \\
& & + \paren{1-\sum_{\substack{i,j\in \mathbb{Z}_{10} \\ i+j\equiv 0 \mod{10}}} p_ip_j }  \Pr_{C=\paren{x_1,\ldots,x_{14}} \sim X_{14}}\left[ f_1\paren{\sigma\paren{C}} = f_1\paren{\sigma '\paren{C}}~\vline ~  \sigma\paren{x_{11}} + \sigma\paren{x_{12}} \nequiv \sigma'\paren{x_{11}}+\sigma'\paren{x_{12}} \mod{10}   \right] \\
&=& \paren{\sum_{\substack{i,j\in \mathbb{Z}_{10}\\i+j\equiv 0 \mod{10}}} p_ip_j } \Pr_{\paren{x_1,x_2,x_{3}} \sim X_{3}}\left[\sum_{i=1}^3 \paren{\sigma\paren{x_i} - \sigma'\paren{x_i}}  \equiv 0 \mod{10} \right] \\
& & + \paren{1-\paren{\sum_{\substack{i,j\in \mathbb{Z}_{10}\\i+j\equiv 0 \mod{10}}} p_ip_j } }  \Pr_{\paren{x,y,x_{13},x_{14}} \sim X_{14}}\left[ \sigma\paren{x}+\sigma\paren{x_{13}} + \sigma\paren{x_{14}} \equiv  \sigma'\paren{y}+\sigma'\paren{x_{13}} + \sigma'\paren{x_{14}} \mod{10} \right] \\
&=& \paren{\sum_{\substack{i,j\in \mathbb{Z}_{10}\\i+j\equiv 0 \mod{10}}} p_ip_j } \Pr_{\paren{x_1,x_2,x_{3}} \sim X_{3}}\paren{\sum_{i,j,k\in \mathbb{Z}_{10}:i+j+k\equiv 0 \mod{10}} p_ip_jp_k }\\
& & + \paren{1-\paren{\sum_{\substack{i,j\in \mathbb{Z}_{10}\\i+j\equiv 0 \mod{10}}} p_ip_j } }  \Pr_{\paren{x,y,x_{13},x_{14}} \sim X_{14}}\left[ \sigma\paren{x}+\sigma\paren{x_{13}} + \sigma\paren{x_{14}} \equiv  \sigma'\paren{y}+\sigma'\paren{x_{13}} + \sigma'\paren{x_{14}} \mod{10} \right] \\
&\leq& \paren{\sum_{\substack{i,j\in \mathbb{Z}_{10}\\i+j\equiv 0 \mod{10}}} p_ip_j } \paren{\sum_{\substack{i,j,k\in \mathbb{Z}_{10}\\i+j+k\equiv 0 \mod{10}}} p_ip_jp_k }\\
& & + \paren{1-\paren{\sum_{\substack{i,j\in \mathbb{Z}_{10}\\i+j\equiv 0 \mod{10}}} p_ip_j } }  
\max_{j\in \mathbb{Z}_{10}} 
\Pr_{\paren{x} \sim [n]}\left[ \sigma\paren{x} \equiv  j \mod{10} \right] \\
&\leq& \paren{\sum_{\substack{i,j\in \mathbb{Z}_{10}\\i+j\equiv 0 \mod{10}}} p_ip_j } \paren{\sum_{\substack{i,j,k\in \mathbb{Z}_{10}\\i+j+k\equiv 0 \mod{10}}} p_ip_jp_k } + \paren{1-\paren{\sum_{\substack{i,j\in \mathbb{Z}_{10}\\i+j\equiv 0 \mod{10}}} p_ip_j } }  \paren{\frac{11}{100}} \\
\end{eqnarray*} 
Maximizing \[\paren{\sum_{\substack{i,j\in \mathbb{Z}_{10}\\i+j\equiv 0 \mod{10}}} p_ip_j } \paren{\sum_{\substack{i,j,k\in \mathbb{Z}_{10}\\i+j+k\equiv 0 \mod{10}}} p_ip_jp_k } + \paren{1-\paren{\sum_{\substack{i,j\in \mathbb{Z}_{10}\\i+j\equiv 0 \mod{10}}} p_ip_j } }  \paren{\frac{11}{100}} \ , \]
subject to the constraint that $p_{0} \leq \frac{1}{10}+\frac{1}{100}$, we obtain the desired upper bound

\[\paren{\sum_{\substack{i,j\in \mathbb{Z}_{10}\\i+j\equiv 0 \mod{10}}} p_ip_j } \paren{\sum_{\substack{i,j,k\in \mathbb{Z}_{10}\\i+j+k\equiv 0 \mod{10}}} p_ip_jp_k } + \paren{1-\paren{\sum_{\substack{i,j\in \mathbb{Z}_{10}\\i+j\equiv 0 \mod{10}}} p_ip_j } }  \paren{\frac{11}{100}} \leq \frac{145}{1000} \ . \]
\end{proofof}

\begin{reminderfact}{\ref{fact:Candidate2Hard}}
\factCandidateTwoHard
\end{reminderfact}

\begin{proofof}{Fact \ref{fact:Candidate2Hard}}
Let $\sigma,\sigma'\in\mathbb{Z}_{10}^n$ be given.   We assume that $\sigma$ is $\paren{\frac{1}{100}}$-balanced and that $\sigma$ and $\sigma'$ are not $\paren{\frac{1}{100}}$-correlated. This means that $\frac{9}{100} \leq \max_{i\in\mathbb{Z}_{10}} \paren{\frac{H\paren{\sigma,\vec{i}}}{n}} \leq \frac{11}{100}$ and   $\paren{1-\frac{H\paren{\sigma,\sigma'}}{n}} < \frac{11}{100}$. It suffices to show that  \[\Pr_{C=\paren{x_1,\ldots,x_{14}} \sim X_{14}}\left[ f_2\paren{\sigma\paren{C}} 
 = f_2\paren{\sigma '\paren{C}} \right] \leq \frac{11}{100} \ . \]

For $j \in \mathbb{Z}_{10}$ we let $p_j = \frac{n-H\paren{\sigma_j,\sigma '}}{n}$ where $\sigma_j\paren{i} = \paren{\sigma\paren{i}+j \mod {10}}$. In particular, $p_{0} = \frac{n-H\paren{\sigma,\sigma '}}{n}$ denotes the probability that $\sigma(i) = \sigma '(i)$ for a random index $i \sim [n]$. By assumption $p_{0} \leq \frac{1}{10}+\frac{1}{100}$. We have

\begin{eqnarray*}
&& \Pr_{C=\paren{x_1,\ldots,x_{14}} \sim X_{14}}\left[ f_2\paren{\sigma\paren{C}} 
 = f_2\paren{\sigma '\paren{C}} \right] \\ &=& \Pr_{C=\paren{x_1,\ldots,x_{14}} \sim X_{14}}\left[ \sigma\paren{x_{11}} = \sigma'\paren{x_{11}} \right] \Pr_{C=\paren{x_1,\ldots,x_{14}} \sim X_{14}}\left[ f_2\paren{\sigma\paren{C}} = f_2\paren{\sigma '\paren{C}}~\vline ~ \sigma\paren{x_{11}} = \sigma'\paren{x_{11}}  \right] \\
& & + \Pr_{C=\paren{x_1,\ldots,x_{14}} \sim X_{14}}\left[ \sigma\paren{x_{11}} \neq \sigma'\paren{x_{11}} \right] \Pr_{C=\paren{x_1,\ldots,x_{14}} \sim X_{14}}\left[ f_2\paren{\sigma\paren{C}} = f_2\paren{\sigma '\paren{C}}~\vline ~ \sigma\paren{x_{11}} \neq \sigma'\paren{x_{11}}  \right] \\
&=& p_{0}\Pr_{C=\paren{x_1,\ldots,x_{14}} \sim X_{14}}\left[ f_2\paren{\sigma\paren{C}} = f_2\paren{\sigma '\paren{C}}~\vline ~ \sigma\paren{x_{11}} = \sigma\paren{x_{11}}  \right] \\
& & + \paren{1-p_{0}}\Pr_{C=\paren{x_1,\ldots,x_{14}} \sim X_{14}}\left[ f_2\paren{\sigma\paren{C}} = f_2\paren{\sigma '\paren{C}}~\vline ~ \sigma\paren{x_{11}} \neq \sigma\paren{x_{11}}  \right] \\
&=& p_{0}\Pr_{C=\paren{x_{12},x_{13},x_{14}} \sim X_{3}}\left[ \sigma\paren{x_{12}} + \ldots + \sigma\paren{x_{14}} \equiv \sigma'\paren{x_{12}} +\ldots + \sigma'\paren{x_{14}} \mod{10}\right] \\
& & + \paren{1-p_{0}}\Pr_{C=\paren{x_1,\ldots,x_{14}} \sim X_{14}}\left[ f_2\paren{\sigma\paren{C}} = f_2\paren{\sigma '\paren{C}}~\vline ~ \sigma\paren{x_{11}} \neq \sigma\paren{x_{11}}  \right] \\
&=& p_{0}\sum_{\substack{i,j,k \in \mathbb{Z}_{10}\\ i+j+k \equiv 0 \mod{10}}} p_ip_jp_k \\
& & + \paren{1-p_{0}}\Pr_{C=\paren{x_1,\ldots,x_{14}} \sim X_{14}}\left[ f_2\paren{\sigma\paren{C}} = f_2\paren{\sigma '\paren{C}}~\vline ~ \sigma\paren{x_{11}} \neq \sigma\paren{x_{11}}  \right] \\
&=& p_{0}\sum_{\substack{i,j,k \in \mathbb{Z}_{10}\\ i+j+k \equiv 0 \mod{10}}} p_ip_jp_k  \\ 
& & + \paren{1-p_{0}}\Pr_{\paren{x,y,x_{12},x_{13},x_{14}} \sim X_{5}}\left[\sigma(x)+\sigma(x_{12})+\sigma\paren{x_{13}}+\sigma\paren{x_{14}} \equiv \sigma'(y)+\sigma'(x_{12})+\sigma'\paren{x_{13}}+\sigma'\paren{x_{14}} \mod{10}  \right] \\
&\leq& p_{0}\sum_{\substack{i,j,k \in \mathbb{Z}_{10}\\ i+j+k \equiv 0 \mod{10}}} p_ip_jp_k  + \paren{1-p_{10}}\max_{j\in\mathbb{Z}_{10}} \Pr_{x \sim [n]}\left[\sigma(x) \equiv j \mod{10}  \right] \\
&\leq& p_{0}\sum_{\substack{i,j,k \in \mathbb{Z}_{10}\\ i+j+k \equiv 0 \mod{10}}} p_ip_jp_k  + \paren{1-p_{10}}\paren{\frac{11}{10}}  \ .
\end{eqnarray*} 
Maximizing \[p_{0}\sum_{\substack{i,j,k \in \mathbb{Z}_{10}\\ i+j+k \equiv 0 \mod{10}}} p_ip_jp_k  + \paren{1-p_{0}}\paren{\frac{11}{10}} \ , \]
subject to the constraint that $p_{0} \leq \frac{1}{10}+\frac{1}{100}$, we obtain the desired upper bound

\[p_{0}\sum_{\substack{i,j,k \in \mathbb{Z}_{10}\\ i+j+k \equiv 0 \mod{10}}} p_ip_jp_k  + \paren{1-p_{0}}\paren{\frac{11}{10}} \leq \frac{11}{100} \ . \]
\end{proofof}

\cut{
\begin{reminderfact}{\ref{fact:Candidate1Hard}}
\factCandidateOneIsHard
\end{reminderfact}

\begin{proofof}{Fact \ref{fact:Candidate1Hard}}
Let $\sigma,\sigma'\in \mathbb{Z}_{10}^n$ be given.  We assume that $\sigma$ is $\paren{\frac{1}{100}}$-balanced and that $\sigma$ and $\sigma'$ are not $\paren{\frac{1}{100}}$-correlated. This means that $\frac{9}{100} \leq \max_{i\in \mathbb{Z}_{10}} \paren{n-\frac{H\paren{\sigma,\vec{i}}}{n}} \leq \frac{11}{100}$ and   $\paren{1-\frac{H\paren{\sigma,\sigma'}}{n}} < \frac{11}{100}$. It suffices to show that  \[\Pr_{C=\paren{x_1,\ldots,x_{14}} \sim X_{14}}\left[ f\paren{\sigma\paren{C}} 
 = f\paren{\sigma '\paren{C}} \right] \leq \frac{145}{1000} \ . \]

For $j \in \mathbb{Z}_{10}$ we let $p_j = \frac{n-H\paren{\sigma_j,\sigma '}}{n}$ where $\sigma_j\paren{i} = \paren{\sigma\paren{i}+j \mod {10}}$. In particular, $p_{0} = \frac{n-H\paren{\sigma,\sigma '}}{n}$ denotes the probability that $\sigma(i) = \sigma '(i)$ for a random index $i \sim [n]$. By assumption $p_{0} \leq \frac{1}{10}+\frac{1}{100}$. We have

\begin{eqnarray*}
&& \Pr_{C=\paren{x_1,\ldots,x_{14}} \sim X_{14}}\left[ f_1\paren{\sigma\paren{C}} 
 = f_1\paren{\sigma '\paren{C}} \right] \\ &=& \paren{\sum_{\substack{i,j\in \mathbb{Z}_{10} \\ i+j\equiv 0 \mod{10}}} p_ip_j } \Pr_{C=\paren{x_1,\ldots,x_{14}} \sim X_{14}}\left[ f_1\paren{\sigma\paren{C}} = f_1\paren{\sigma '\paren{C}}~\vline ~  \sigma\paren{x_{11}} + \sigma\paren{x_{12}} \equiv \sigma'\paren{x_{11}}+\sigma'\paren{x_{12}} \mod{10}  \right] \\
& & + \paren{1-\sum_{\substack{i,j\in \mathbb{Z}_{10} \\ i+j\equiv 0 \mod{10}}} p_ip_j }  \Pr_{C=\paren{x_1,\ldots,x_{14}} \sim X_{14}}\left[ f_1\paren{\sigma\paren{C}} = f_1\paren{\sigma '\paren{C}}~\vline ~  \sigma\paren{x_{11}} + \sigma\paren{x_{12}} \nequiv \sigma'\paren{x_{11}}+\sigma'\paren{x_{12}} \mod{10}   \right] \\
&=& \paren{\sum_{\substack{i,j\in \mathbb{Z}_{10}\\i+j\equiv 0 \mod{10}}} p_ip_j } \Pr_{\paren{x_1,x_2,x_{3}} \sim X_{3}}\left[\sum_{i=1}^3 \paren{\sigma\paren{x_i} - \sigma'\paren{x_i}}  \equiv 0 \mod{10} \right] \\
& & + \paren{1-\paren{\sum_{\substack{i,j\in \mathbb{Z}_{10}\\i+j\equiv 0 \mod{10}}} p_ip_j } }  \Pr_{\paren{x,y,x_{13},x_{14}} \sim X_{14}}\left[ \sigma\paren{x}+\sigma\paren{x_{13}} + \sigma\paren{x_{14}} \equiv  \sigma'\paren{y}+\sigma'\paren{x_{13}} + \sigma'\paren{x_{14}} \mod{10} \right] \\
&=& \paren{\sum_{\substack{i,j\in \mathbb{Z}_{10}\\i+j\equiv 0 \mod{10}}} p_ip_j } \Pr_{\paren{x_1,x_2,x_{3}} \sim X_{3}}\paren{\sum_{i,j,k\in \mathbb{Z}_{10}:i+j+k\equiv 0 \mod{10}} p_ip_jp_k }\\
& & + \paren{1-\paren{\sum_{\substack{i,j\in \mathbb{Z}_{10}\\i+j\equiv 0 \mod{10}}} p_ip_j } }  \Pr_{\paren{x,y,x_{13},x_{14}} \sim X_{14}}\left[ \sigma\paren{x}+\sigma\paren{x_{13}} + \sigma\paren{x_{14}} \equiv  \sigma'\paren{y}+\sigma'\paren{x_{13}} + \sigma'\paren{x_{14}} \mod{10} \right] \\
&\leq& \paren{\sum_{\substack{i,j\in \mathbb{Z}_{10}\\i+j\equiv 0 \mod{10}}} p_ip_j } \paren{\sum_{\substack{i,j,k\in \mathbb{Z}_{10}\\i+j+k\equiv 0 \mod{10}}} p_ip_jp_k }\\
& & + \paren{1-\paren{\sum_{\substack{i,j\in \mathbb{Z}_{10}\\i+j\equiv 0 \mod{10}}} p_ip_j } }  
\max_{j\in \mathbb{Z}_{10}} 
\Pr_{\paren{x} \sim [n]}\left[ \sigma\paren{x} \equiv  j \mod{10} \right] \\
&\leq& \paren{\sum_{\substack{i,j\in \mathbb{Z}_{10}\\i+j\equiv 0 \mod{10}}} p_ip_j } \paren{\sum_{\substack{i,j,k\in \mathbb{Z}_{10}\\i+j+k\equiv 0 \mod{10}}} p_ip_jp_k } + \paren{1-\paren{\sum_{\substack{i,j\in \mathbb{Z}_{10}\\i+j\equiv 0 \mod{10}}} p_ip_j } }  \paren{\frac{11}{100}} \\
\end{eqnarray*} 
Maximizing \[\paren{\sum_{\substack{i,j\in \mathbb{Z}_{10}\\i+j\equiv 0 \mod{10}}} p_ip_j } \paren{\sum_{\substack{i,j,k\in \mathbb{Z}_{10}\\i+j+k\equiv 0 \mod{10}}} p_ip_jp_k } + \paren{1-\paren{\sum_{\substack{i,j\in \mathbb{Z}_{10}\\i+j\equiv 0 \mod{10}}} p_ip_j } }  \paren{\frac{11}{100}} \ , \]
subject to the constraint that $p_{0} \leq \frac{1}{10}+\frac{1}{100}$, we obtain the desired upper bound

\[\paren{\sum_{\substack{i,j\in \mathbb{Z}_{10}\\i+j\equiv 0 \mod{10}}} p_ip_j } \paren{\sum_{\substack{i,j,k\in \mathbb{Z}_{10}\\i+j+k\equiv 0 \mod{10}}} p_ip_jp_k } + \paren{1-\paren{\sum_{\substack{i,j\in \mathbb{Z}_{10}\\i+j\equiv 0 \mod{10}}} p_ip_j } }  \paren{\frac{11}{100}} \leq \frac{145}{1000} \ . \]
\end{proofof}

\begin{reminderfact}{\ref{fact:Candidate2Hard}}
\factCandidateTwoHard
\end{reminderfact}

\begin{proofof}{Fact \ref{fact:Candidate2Hard}}
Let $\sigma,\sigma'\in\mathbb{Z}_{10}^n$ be given.   We assume that $\sigma$ is $\paren{\frac{1}{100}}$-balanced and that $\sigma$ and $\sigma'$ are not $\paren{\frac{1}{100}}$-correlated. This means that $\frac{9}{100} \leq \max_{i\in\mathbb{Z}_{10}} \paren{\frac{H\paren{\sigma,\vec{i}}}{n}} \leq \frac{11}{100}$ and   $\paren{1-\frac{H\paren{\sigma,\sigma'}}{n}} < \frac{11}{100}$. It suffices to show that  \[\Pr_{C=\paren{x_1,\ldots,x_{14}} \sim X_{14}}\left[ f_2\paren{\sigma\paren{C}} 
 = f_2\paren{\sigma '\paren{C}} \right] \leq \frac{11}{100} \ . \]

For $j \in \mathbb{Z}_{10}$ we let $p_j = \frac{n-H\paren{\sigma_j,\sigma '}}{n}$ where $\sigma_j\paren{i} = \paren{\sigma\paren{i}+j \mod {10}}$. In particular, $p_{0} = \frac{n-H\paren{\sigma,\sigma '}}{n}$ denotes the probability that $\sigma(i) = \sigma '(i)$ for a random index $i \sim [n]$. By assumption $p_{0} \leq \frac{1}{10}+\frac{1}{100}$. We have

\begin{eqnarray*}
&& \Pr_{C=\paren{x_1,\ldots,x_{14}} \sim X_{14}}\left[ f_2\paren{\sigma\paren{C}} 
 = f_2\paren{\sigma '\paren{C}} \right] \\ &=& \Pr_{C=\paren{x_1,\ldots,x_{14}} \sim X_{14}}\left[ \sigma\paren{x_{11}} = \sigma'\paren{x_{11}} \right] \Pr_{C=\paren{x_1,\ldots,x_{14}} \sim X_{14}}\left[ f_2\paren{\sigma\paren{C}} = f_2\paren{\sigma '\paren{C}}~\vline ~ \sigma\paren{x_{11}} = \sigma'\paren{x_{11}}  \right] \\
& & + \Pr_{C=\paren{x_1,\ldots,x_{14}} \sim X_{14}}\left[ \sigma\paren{x_{11}} \neq \sigma'\paren{x_{11}} \right] \Pr_{C=\paren{x_1,\ldots,x_{14}} \sim X_{14}}\left[ f_2\paren{\sigma\paren{C}} = f_2\paren{\sigma '\paren{C}}~\vline ~ \sigma\paren{x_{11}} \neq \sigma'\paren{x_{11}}  \right] \\
&=& p_{0}\Pr_{C=\paren{x_1,\ldots,x_{14}} \sim X_{14}}\left[ f_2\paren{\sigma\paren{C}} = f_2\paren{\sigma '\paren{C}}~\vline ~ \sigma\paren{x_{11}} = \sigma\paren{x_{11}}  \right] \\
& & + \paren{1-p_{0}}\Pr_{C=\paren{x_1,\ldots,x_{14}} \sim X_{14}}\left[ f_2\paren{\sigma\paren{C}} = f_2\paren{\sigma '\paren{C}}~\vline ~ \sigma\paren{x_{11}} \neq \sigma\paren{x_{11}}  \right] \\
&=& p_{0}\Pr_{C=\paren{x_{12},x_{13},x_{14}} \sim X_{3}}\left[ \sigma\paren{x_{12}} + \ldots + \sigma\paren{x_{14}} \equiv \sigma'\paren{x_{12}} +\ldots + \sigma'\paren{x_{14}} \mod{10}\right] \\
& & + \paren{1-p_{0}}\Pr_{C=\paren{x_1,\ldots,x_{14}} \sim X_{14}}\left[ f_2\paren{\sigma\paren{C}} = f_2\paren{\sigma '\paren{C}}~\vline ~ \sigma\paren{x_{11}} \neq \sigma\paren{x_{11}}  \right] \\
&=& p_{0}\sum_{\substack{i,j,k \in \mathbb{Z}_{10}\\ i+j+k \equiv 0 \mod{10}}} p_ip_jp_k \\
& & + \paren{1-p_{0}}\Pr_{C=\paren{x_1,\ldots,x_{14}} \sim X_{14}}\left[ f_2\paren{\sigma\paren{C}} = f_2\paren{\sigma '\paren{C}}~\vline ~ \sigma\paren{x_{11}} \neq \sigma\paren{x_{11}}  \right] \\
&=& p_{0}\sum_{\substack{i,j,k \in \mathbb{Z}_{10}\\ i+j+k \equiv 0 \mod{10}}} p_ip_jp_k  \\ 
& & + \paren{1-p_{0}}\Pr_{\paren{x,y,x_{12},x_{13},x_{14}} \sim X_{5}}\left[\sigma(x)+\sigma(x_{12})+\sigma\paren{x_{13}}+\sigma\paren{x_{14}} \equiv \sigma'(y)+\sigma'(x_{12})+\sigma'\paren{x_{13}}+\sigma'\paren{x_{14}} \mod{10}  \right] \\
&\leq& p_{0}\sum_{\substack{i,j,k \in \mathbb{Z}_{10}\\ i+j+k \equiv 0 \mod{10}}} p_ip_jp_k  + \paren{1-p_{10}}\max_{j\in\mathbb{Z}_{10}} \Pr_{x \sim [n]}\left[\sigma(x) \equiv j \mod{10}  \right] \\
&\leq& p_{0}\sum_{\substack{i,j,k \in \mathbb{Z}_{10}\\ i+j+k \equiv 0 \mod{10}}} p_ip_jp_k  + \paren{1-p_{10}}\paren{\frac{11}{10}}  \ .
\end{eqnarray*} 
Maximizing \[p_{0}\sum_{\substack{i,j,k \in \mathbb{Z}_{10}\\ i+j+k \equiv 0 \mod{10}}} p_ip_jp_k  + \paren{1-p_{0}}\paren{\frac{11}{10}} \ , \]
subject to the constraint that $p_{0} \leq \frac{1}{10}+\frac{1}{100}$, we obtain the desired upper bound

\[p_{0}\sum_{\substack{i,j,k \in \mathbb{Z}_{10}\\ i+j+k \equiv 0 \mod{10}}} p_ip_jp_k  + \paren{1-p_{0}}\paren{\frac{11}{10}} \leq \frac{11}{100} \ . \]
\end{proofof}}
\cut{
\begin{reminderclaim}{\ref{claim:FamilyIsHardToPredict}}
\claimFamilyIsHardToPredict
\end{reminderclaim}
\begin{proofof}{Claim \ref{claim:FamilyIsHardToPredict}}
Let $\sigma, \sigma' \in \mathbb{Z}_d^n$ be given such that $\tau= \paren{\sigma - \sigma'}$ is $\delta$--balanced. Let $k = k_1+k_2+10$. Given $C = \paren{i_1,\ldots,i_k} \in X_k$ we write $C^{-1} \doteq \paren{i_1,\ldots,i_{k-1}}$. We observe that 
\[ f_{k_1,k_2}\paren{\sigma\paren{C}} = f_{k_1,k_2-1}\paren{\sigma\paren{{C^{-1}}}} +\sigma\paren{i_k} \mod{10} \ .\]
If we have $f_{k_1,k_2}\paren{\sigma\paren{C}} = f_{k_1,k_2}\paren{\sigma'\paren{C}}$ then we must have 
\[ \sigma\paren{i_k}-\sigma'\paren{i_k} \equiv f_{k_1,k_2-1}\paren{\sigma'\paren{C^{-1}}}-f_{k_1,k_2-1}\paren{\sigma\paren{C^{-1}}} \mod{10} \ .\]
 If we let $\mathbf{EQ}\paren{C^{-1},j}$ denote the event that $j = f_{k_1,k_2-1}\paren{\sigma'\paren{C^{-1}}}-f_{k_1,k_2-1}\paren{\sigma\paren{C^{-1}}} \mod{10}$ then
\begin{eqnarray*}
 &  &  \Pr_{C=\paren{i_1,\ldots,i_{k_1+k_2+10}} \sim X_{k_1+k_2+10}}\left[f_{k_1,k_2}\paren{\sigma\paren{C}} = f_{k_1,k_2} \paren{\sigma'\paren{C}} \right] ~~~~~~~~~~~~~ \\ & \leq &  \max_{0 \leq j \leq 9} \Pr_{C=\paren{i_1,\ldots,i_{k_1+k_2+10}\sim X_k}}\left[ \tau\paren{i_k} \equiv j \mod{10} ~\vline~\mathbf{EQ}\paren{C^{-1},j}\right]\\
 &\leq& \frac{1}{d}+\delta+\frac{k-1}{n}   \ ,
\end{eqnarray*} 
where the last line follows because $\tau$ is $\delta$--balanced.
\end{proofof}}

